A Fully-Configurable Open-Source Software-Defined Digital Quantized Spiking Neural Core Architecture

We introduce QUANTISENC, a fully configurable open-source software-defined digital quantized spiking neural core architecture to advance research in neuromorphic computing. QUANTISENC is designed hierarchically using a bottom-up methodology with multiple neurons in each layer and multiple layers in each core. The number of layers and neurons per layer can be configured via software in a top-down methodology to generate the hardware for a target spiking neural network (SNN) model. QUANTISENC uses leaky integrate and fire neurons (LIF) and current-based excitatory and inhibitory synapses (CUBA). The nonlinear dynamics of a neuron can be configured at run-time via programming its internal control registers. Each neuron performs signed fixed-point arithmetic with user-defined quantization and decimal precision. QUANTISENC supports all-to-all, one-to-one, and Gaussian connections between layers. Its hardware-software interface is integrated with a PyTorch-based SNN simulator. This integration allows to define and train an SNN model in PyTorch and evaluate the hardware performance (e.g., area, power, latency, and throughput) through FPGA prototyping and ASIC design. The hardware-software interface also takes advantage of the layer-based architecture and distributed memory organization of QUANTISENC to enable pipelining by overlapping computations on streaming data. Overall, the proposed software-defined hardware design methodology offers flexibility similar to that of high-level synthesis (HLS), but provides better hardware performance with zero hardware development effort. We evaluate QUANTISENC using three spiking datasets and show its superior performance against state-of the-art designs.

==> sections/edu.tex <==
Figure~\ref{fig:edu} describes at a high level the curriculum that integrates \tech{} to educate students in the Department of Electrical and Computer Engineering (ECE) of Drexel University.
%The three digit number in each block refers to the identifier in our course catalog.
The curriculum is structured into undergraduate and graduate contents.
At the undergraduate level, students are introduced to machine learning (ML) engineering based on the fundamentals of probability and data analytics. 
Student projects involve ML training and inference using the Python-based PyTorch framework.
The introduction to VLSI course introduces HDL coding using the Verilog HDL language with digital logic as background. 
Student projects include designing adders and multipliers in Verilog and verifying them using testbenches.
On the analog front, courses such as electronic devices introduce students to the basics of semiconductors. Thereafter, the modern transistor design course introduces CMOS technology. 
Student projects in this course involve designing adder circuitry using CMOS transistors.

\begin{figure}[h!]
    \centering
    \centerline{\includegraphics[width=0.99\columnwidth]{images/education.pdf}}
    \caption{Educational curriculum integrating \tech{}.}
    \label{fig:edu}
\end{figure}

At the graduate level, the Machine Learning and AI course covers the mathematical foundation of AI and also introduces different deep learning models. 
The system neuroscience course is an interdisciplinary course that introduces the neuronal and circuit basis underlying sensory processing and perception. 
This course also introduces the Spiking Neural Network (SNN) using simple neuron and synapse models.

On the hardware front, the introduction to the VLSI course at the undergraduate level leads to ASIC and FPGA design courses, which form the prerequisite to the neuromorphic computing course. 
For the ASIC design course, we plan to use \tech{} as a design reference to introduce the design and automation of digital CMOS Application Specific Integrated Circuit (ASIC) systems.
The ASIC physical design flow, including logic synthesis, floorplanning, placement, clock tree synthesis, routing, and verification will be presented. These back-end physical design flow steps will also be covered through hands-on practice using industrial VLSI CAD tools.

The project-based digital FPGA design course will teach students how to implement \tech{} on the Xilinx FPGA.
Students will learn to perform simulations using the testbench.
Students will also learn to analyze design rule check (DRC) violations and design closure for \tech{}-based intellectual property (IP) design and management.

\begin{figure*}[h!]
    \centering
    \centerline{\includegraphics[width=1.99\columnwidth]{images/256x128x10.pdf}}
    \caption{A classification example with the spiking MNIST dataset using the handwritten digit 8. \tech{} is configured as a $256\times 128\times 10$ architecture.}
    \label{fig:example_8}
\end{figure*}

The neuromorphic computing course will utilize all key concepts in prerequisite courses to introduce hardware-software co-design in the area of AI.
The course is structured into three sections.
In the first section, the course will introduce key concepts in SNNs, including different types of neuron and synapse, and learning approaches using SNNs, e.g., supervised, unsupervised, and reinforcement learning.
The projects in this section will include developing time series and image-based applications using SNNs.
In the second section, the course will introduce \tech{} hardware and its implementation on FPGA.
The projects will include extending \tech{} to support different neuron models, exploring the trade-off in hardware and software performance. 
The third section of this course is planned to be project-based, where students will learn the end-to-end implementation of neuromorphic systems for target applications.



The neuromorphic computing course will form the prerequisite for a full-stack co-design oriented course that will 
integrate \textit{all} compute stacks into the curriculum, teaching students to explore design points that span these stacks. 
The proposed course will facilitate both a \textbf{top-down understanding}, where new(er) applications can create the need for architectural features/assists, which in turn can drive innovations in circuits leveraging and optimizing newer materials/devices, and a \textbf{bottom-up understanding}, where novel material/device features and challenges can open up new architectural features that can enable/enhance new(er) applications.


This educational curriculum addresses the specific need to build a robust semiconductor workforce that specializes in AI systems.
In the future, we plan to extend this curriculum structure to add courses that address heterogeneous integration of CMOS and emerging non-volatile memory technologies.

% development and of designing specialized heterogeneous systems integrating CMOS and emerging memory technologies as a path forward to technology scaling limits. Our focus is on artificial intelligence (AI) systems and we aim to co-design the compute stacks for such systems tailored to on-chip learning via neuromorphic computing, which is a mechanism to learn from a constant stream of data, much like humans do, and adapt its decisions when necessary.

% Finally, the EDA course introduces the key steps in electronic design automation (EDA) using \tech{} as the target design.
% This project based course introduces backend flow including  floorplanning, placement, clock tree synthesis, and routing.
% This course will involve a fabrication component in the future to fabricate \tech{} on silicon.

% The proposed curriculum structure addresses two key areas -- (1) a lack of robust semiconductor workforce and (2) a lack of proper mechanisms to transition innovations from lab to fab. 
% In the future, we plan to extend this curriculum structure to also include course that addresses heterogeneous integration of CMOS and emerging non-volatile memory technologies.

==> sections/extra.tex <==
Although high-level synthesis (HLS) using commercial tools such as Vitis~\cite{kathail2020xilinx} and academic platforms such as Bambu~\cite{ferrandi2021bambu} can generate hardware description language (HDL) starting from a software specification, there are four key limitations of neuromorphic HLS that we address in this work. 
First, the HDL generated from HLS is not parameterizable. 
Therefore, any change in software description requires regenerating its HDL using the HLS flow, as illustrated in Figure~\ref{fig:compare}a. 
Large run times prohibit the use of HLS flow inside a co-design loop, where several hundred iterations may be necessary to achieve the required hardware and software performance for a target SNN model.
Second, most HLS tools do not support neuromorphic computations, and those that do support require a significant amount of engineering effort at the kernel level for compilation and mapping, in addition to the effort needed in hardware development to add new computations or extend existing ones, as shown in our recent work~\cite{iccad2021b}.
Third, most HLS tools work with dataflow graphs extracted from machine learning applications and perform static scheduling on them, exploiting only batch-level hardware parallelism. 
\footnote{A batch-level parallelism is a type of parallel computing environment in a neuromorphic hardware where multiple batches of input data are processed concurrently on different processing elements~\cite{memocode2022}.}
There remains a significant opportunity to improve performance, such as throughput, by taking advantage of other forms of parallelism that are present in neuromorphic hardware.
Finally, the HDL generated from HLS is not always hardware efficient, as shown in several previous works~\cite{liu2022overgen,cong2022fpga,ahangari2023hls}.



\textbf{Contribution --} We introduce \tech{}, a fully configurable open-source software-defined digital neuromorphic architecture to advance research and education in AI hardware.
Figure~\ref{fig:compare}b shows our design methodology.
\tech{} can be tailored to match the exact specification of a user code (application software) simply by changing the following two sets of design parameters.
\begin{itemize}
    \item \textbf{Static Parameters:} These are design parameters that are configured at design-time to define the model structure and its quantization. The static parameters of \tech{} are the number of layers (\texttt{layers}), neurons-per-layer (\texttt{neurons}), layer-to-layer connectivity (\texttt{connect}), and 
    precision for synaptic weights and state variables (\texttt{precision}).
    \item \textbf{Dynamic Parameters:} These are design parameters that are configured at run-time by programming its internal control registers via the system software (OS). The dynamic parameters of \tech{} are neuron parameters (\texttt{params}) and neuron dynamics (\texttt{dynamics}).
    These parameters are elaborated in Section~\ref{sec:lif}.
\end{itemize}

\begin{figure}[h!]
    \centering
    \centerline{\includegraphics[width=0.99\columnwidth]{images/compare_v4.pdf}}
    \caption{(a) A High-Level Synthesis (HLS) flow within a co-design loop. (b) Our design methodology integrating \tech{} within a co-design loop.}
    \label{fig:compare}
\end{figure}

\tech{} is designed to work with PyTorch-based SNN simulators such as SNNTorch~\cite{chollet2021deep} and SpikingJelly~\cite{spikingjelly}.
Our code generation library can be imported into a user's code to configure \tech{} and generate a SystemVerilog testbench (\texttt{tb}) to perform behavioral, functional, and timing verification of \tech{}.
This fully automated design flow from model specification in software to hardware design and verification
is the core of our hardware-software co-design, as illustrated in Figure~\ref{fig:compare}b.
Our co-design flow does not require optimization at the kernel level, unlike an HLS.
This reduces the time to evaluate each design refinement, which reduces the overall co-design time (see Section~\ref{sec:results}).

\tech{} cores can be integrated with a shared interconnect such as the segmented bus~\cite{tetc2023} and Network-on-Chip (NoC)~\cite{liu2018neu} to build large-scale neuromorphic hardware~\cite{date2022}.
Although there are other layer-based architectures such as \ub{}~\cite{stuijt2021mubrain} and Gyro~\cite{corradi2021gyro},
\tech{} differs from them in the following four aspects.

==> sections/introduction_bk.tex <==


\IEEEPARstart{N}{euromorphic} computing describes the hardware implementation of biological nervous systems~\cite{mead1990neuromorphic}.
Since this original work, architects and designers have created brain-like processing systems using analog and digital components. 
These architectures offer lower power consumption, reduced latencies, and many other benefits seen in biological systems.
Although analog designs can take advantage of electronic and physical laws in implementing neurons and synapses, which make them energy efficient, digital designs are faster to implement due to the maturity of their design flow and can take advantage of the technology scaling~\cite{joubert2012hardware}. 

Existing digital designs suffer from the following three key limitations, which we address in this work.
First, once implemented on silicon, existing digital designs allow only programming of its synaptic weights. 
They do not allow for configuring the neuron dynamics at run-time.
We show that the run-time configuration can be used to explore the trade-off between performance and power (Section~\ref{sec:dynamic}). 
Second, existing designs lack a well-defined hardware-software interface to stream input, visualize output, and load design configurations and synaptic weights.
We show that a hardware-software interface can also be used to allow pipelining to improve performance (Section~\ref{sec:throughput}).
Finally, no existing digital designs are available as open-source release.
We believe that open-source hardware designs can rapidly advance both research and education in neuromorphic computing (Section~\ref{sec:edu}). 

%-- (1) lack of design configurability, (2) lack of a hardware-software
%First, most designs do not support 

We propose a fully configurable layer-based neuromorphic hardware design and its design methodology in which the number of layers, neurons per layer, layer-to-layer connectivity, neuron parameters, nonlinear neuron dynamics, quantization, and decimal precision can be configured through software to generate the hardware for spiking neural networks (SNNs)~\cite{maass1997networks}. 
%From a research perspective, 
This software-defined hardware design methodology allows researchers and system designers to train an SNN model in software (e.g., Python) and evaluate its hardware performance, such as area, power, latency, and throughput through FPGA prototyping and ASIC design.
The proposed methodology can also be used to teach digital neuromorphic design to STEM students using the widely-used Python language, focusing on the key area of artificial intelligence (AI).
%The digital design generated by using our methodology can benefit from the maturity of microelectronic process technology by reducing the time-to-market of neuromorphic products.

% From an education perspective, given the ubiquity of Python and its perpetually increasing integration into K-12 education, our goal is to develop a Python-based framework that can be used to teach digital design to STEM students, focusing on the key area of artificial intelligence (AI).
% Using this framework, students can learn biology-inspired AI and evaluate trade-offs involved in making specific design choices while performing application-hardware co-design of AI systems.

\IEEEpubidadjcol

Although high-level synthesis (HLS) using commercial tools such as Vitis~\cite{kathail2020xilinx} and academic platforms such as Bambu~\cite{ferrandi2021bambu} can generate hardware description language (HDL) starting from a software specification, there are four key limitations of neuromorphic HLS that we address in this work. 
First, the HDL generated from HLS is not parameterizable. 
Therefore, any change in software description requires regenerating its HDL using the HLS flow, as illustrated in Figure~\ref{fig:compare}a. 
Large run times prohibit the use of HLS flow inside a co-design loop, where several hundred iterations may be necessary to achieve the required hardware and software performance for a target SNN model.
Second, most HLS tools do not support neuromorphic computations, and those that do support require a significant amount of engineering effort at the kernel level for compilation and mapping, in addition to the effort needed in hardware development to add new computations or extend existing ones, as shown in our recent work~\cite{iccad2021b}.
Third, most HLS tools work with dataflow graphs extracted from machine learning applications and perform static scheduling on them, exploiting only batch-level hardware parallelism. 
\footnote{A batch-level parallelism is a type of parallel computing environment in a neuromorphic hardware where multiple batches of input data are processed concurrently on different processing elements~\cite{memocode2022}.}
There remains a significant opportunity to improve performance, such as throughput, by taking advantage of other forms of parallelism that are present in neuromorphic hardware.
Finally, the HDL generated from HLS is not always hardware-efficient, as shown in several previous works~\cite{liu2022overgen,cong2022fpga,ahangari2023hls}.



\textbf{Contribution --} We introduce \tech{}, a fully configurable open-source software-defined digital neuromorphic architecture to advance research and education in AI hardware.
Figure~\ref{fig:compare}b shows our design methodology.
\tech{} can be tailored to match the exact specification of a user code (application software) simply by changing the following two sets of design parameters.
\begin{itemize}
    \item \textbf{Static Parameters:} These are design parameters that are configured at design-time to define the model structure and its quantization. The static parameters of \tech{} are the number of layers (\texttt{layers}), neurons-per-layer (\texttt{neurons}), layer-to-layer connectivity (\texttt{connect}), and 
    precision for synaptic weights and state variables (\texttt{precision}).
    \item \textbf{Dynamic Parameters:} These are design parameters that are configured at run-time by programming its internal control registers via the system software (OS). The dynamic parameters of \tech{} are neuron parameters (\texttt{params}) and neuron dynamics (\texttt{dynamics}).
    These parameters are elaborated in Section~\ref{sec:lif}.
\end{itemize}

\begin{figure}[h!]
    \centering
    \centerline{\includegraphics[width=0.99\columnwidth]{images/compare_v4.pdf}}
    \caption{(a) A High-Level Synthesis (HLS) flow within a co-design loop. (b) Our design methodology integrating \tech{} within a co-design loop.}
    \label{fig:compare}
\end{figure}

\tech{} is designed to work with PyTorch-based SNN simulators such as SNNTorch~\cite{chollet2021deep} and SpikingJelly~\cite{spikingjelly}.
Our code generation library can be imported into a user's code to configure \tech{} and generate a SystemVerilog testbench (\texttt{tb}) to perform behavioral, functional, and timing verification of \tech{}.
This fully automated design flow from model specification in software to hardware design and its verification
is the core of our hardware-software co-design, as illustrated in Figure~\ref{fig:compare}b.
Our co-design flow does not require optimization at the kernel level, unlike an HLS.
This reduces the time to evaluate each design refinement, which reduces the overall co-design time (see Section~\ref{sec:results}).

\tech{} cores can be integrated with a shared interconnect such as the segmented bus~\cite{tetc2023} and Network-on-Chip (NoC)~\cite{liu2018neu} to build large-scale neuromorphic hardware~\cite{date2022}.
Although there are other layer-based architectures such as \ub{}~\cite{stuijt2021mubrain} and Gyro~\cite{corradi2021gyro},
\tech{} differs from them in the following four aspects.
\begin{enumerate}
    \item \textbf{Configurable:} 
    \tech{} is designed hierarchically in a bottom-up methodology with neurons, layers, and cores. The number of layers and neurons per layer can be configured by software in a top-down methodology to generate hardware for a target SNN model.
    \tech{} supports signed computations of fixed-point arithmetic with user-defined precision and quantization.
    Currently, \tech{} implements leaky integrate-and-fire neurons (LIF)~\cite{indiveri2003low}, and current-based excitatory and inhibitory synapses (CUBA), with all-to-all, one-to-one, and Gaussian connections between layers. 
    Using our modular design methodology, \tech{} can be easily extended to support other types of neurons, e.g., Izhikevich and compartmental~\cite{ward2022beyond}, and synapse, e.g., conductance-based synapse (COBA)~\cite{cessac2008dynamics}.
    \item \textbf{Hardware-Software Interface:}
    A key novelty of our design methodology is that it allows the LIF parameters and LIF dynamics to be configured from an application software (e.g., PyTorch code) at runtime by programming the internal control registers on the hardware through its interface with the system software (OS), as illustrated in Figure~\ref{fig:compare}b.
    This gives the user additional flexibility to fine-tune hardware performance after the design has been fabricated on silicon.
    Our hardware-software interface is also used to program synaptic weights, drive input, and visualize hardware output.
    \item \textbf{Pipelining:} \tech{} implements a distributed memory organization, where the synaptic memory of neurons in a layer is instantiated within each layer, allowing the layers of \tech{} to operate independently and parallel to each other.
    Although \tech{} is a dataflow architecture with layer-by-layer processing of input data, we leverage the parallelism in its internal layer design by overlapping the processing of streaming data in a pipelined fashion using the proposed hardware-software interface.
    This refinement of dataflow computations significantly improves the throughput.

    \item \textbf{Open-Source Release:} \tech{} is developed over a period of eight years and is supported by Accenture LLP, three US National Science Foundation research grants, one US Department of Energy grant, and one European Horizon 2020 research grant.
    \tech{} is developed to foster future research and education in neuromorphic computing.
    \tech{} will be released under the open-source MIT license, which allows academia and industry to access the design without restriction.
    The direct link to the code and its extensive documentation is provided here for review purposes.\footnote{\url{https://www.anupkdas.com}}
    Upon acceptance, this link will be replaced by the GitHub access link. 
\end{enumerate}

\begin{figure*}[t!]
    \centering
    \centerline{\includegraphics[width=1.5\columnwidth]{images/quantisenc_v7.pdf}}
    \caption{(a) High-level overview of \tech{'s} design blocks. (b) Computation of spike trains using synaptic weights.}
    \label{fig:snncore}
\end{figure*}

We evaluated \tech{} and our system design methodology using DVS Gesture~\cite{amir2017low}, MNIST~\cite{fatahi2016evt_mnist}, and Spiking Heidelberg Digit (SHD)~\cite{cramer2020heidelberg} datasets.
Our results show that compared to the software implementation, the hardware implementation of LIF dynamics has a mean square error (MSE) of only \textcolor{red}{x\%} with a precision of \textcolor{red}{n} bits for synaptic weights and state variables. 
The MSE reduces to \textcolor{red}{y\%}, when the precision is increased to \textcolor{red}{m} bits. 
For dataset results, \tech{} significantly outperforms state-of-the-art designs in terms of resource utilization, power, latency, and throughput. 
We show the scalability of \tech{} for different datasets and settings of its design parameters.
